MaskGIT: Masked Generative Image Transformer

Generative transformers have experienced rapid popularity growth in the computer vision community in synthesizing high-fidelity and high-resolution images. The best generative transformer models so far, however, still treat an image naively as a sequence of tokens, and decode an image sequentially following the raster scan ordering (i.e. line-by-line). We find this strategy neither optimal nor efficient. This paper proposes a novel image synthesis paradigm using a bidirectional transformer decoder, which we term MaskGIT. During training, MaskGIT learns to predict randomly masked tokens by attending to tokens in all directions. At inference time, the model begins with generating all tokens of an image simultaneously, and then refines the image iteratively conditioned on the previous generation. Our experiments demonstrate that MaskGIT significantly outperforms the state-of-the-art transformer model on the ImageNet dataset, and accelerates autoregressive decoding by up to 64x. Besides, we illustrate that MaskGIT can be easily extended to various image editing tasks, such as inpainting, extrapolation, and image manipulation.

==> figures/ablation.tex <==
\setlength{\tabcolsep}{5pt}

\begin{table}[!ht]
\small
    \centering
    {\small
    \resizebox{0.7\linewidth}{!}{
        \begin{tabular}{lc cccc}
            \toprule
            {\large$\gamma$} &  %\bfseries{Sampling method}  &
              & $T$ & \bfseries{FID}  $\downarrow$ & \bfseries{IS} $\uparrow$ & \bfseries{NLL} \\
            \midrule
            Exponential & 
            & 4  & 20.84 & 69.7 & 5.86 \\
            Cubic & 
            & 9 & 7.26 & 165.2 & 4.63  \\ 
            Square & 
            & 10 & 6.35 & 179.9 & 4.38  \\ 
            \textbf{Cosine} & 
            & 10 & \textbf{6.06} & \textbf{181.5} & 4.22 \\    
            Linear & 
            & 16 & 7.51 & 113.2 & 3.75  \\
            Square Root &
            & 32 & 12.33 & 99.0 & 3.34 \\  
            Logarithmic  &
            & 72 & 26.12 & 46.7 &  3.08\\
    \bottomrule
    \end{tabular}
    }
    }
    \vspace{-.1cm}
    \caption{\textbf{Ablation results on the mask scheduling functions.} We report the best FID, IS, and Negative Log-Likelihood loss for each candidate scheduling function. }
    \label{tab:ablation}
\vspace{-.5cm}
\end{table}


% \begin{figure}[!t]
%     \centering
% \includegraphics[width=0.8\linewidth]{figures/iteration_vs_fid_scheduling_method.pdf}
%     % \vspace{-25mm}
%     \caption{\textbf{\# of iterations \textit{T}}. Each line graphs a model's FID score against the number of refinement iterations. The lines are named as ''\textit{training distribution - refinement schedule}", e.g. "Linear - Cosine" represents the model that is trained with a linear (i.e. uniform) distribution of mask ratios and uses a cosine refinement schedule.}
%     \label{fig:fidschedule}
% \end{figure}

\begin{figure}[!t]
    \centering
\includegraphics[width=1.\linewidth]{figures/scheduling_func.pdf}
    \vspace{-6mm}
    \caption{\textbf{Choices of Mask Scheduling Functions} $\gamma (\frac{t}{T})$, and 
    \textbf{number of iterations \textit{T}}. On the left, we visualize seven functions we consider for $\gamma$. On the right, we show line graphs of models' FID scores against the number of decoding iterations $T$. Among the candidates, we find that cosine achieves the best FID.}
    \label{fig:scheduling}
    \vspace{-5mm}
\end{figure}

==> figures/cas_table.tex <==
\newcolumntype{N}{@{}m{0pt}@{}}

\begin{table*}[h]
\small
    \centering
    {\small
    \begin{tabular}{lc ccc ccc ccc cc}
    \toprule
     {Model} & 
    
     & {FID}  $\downarrow$ & {IS}  $\uparrow$ & 
     &  {Prec}  $\uparrow$ & {Rec}   $\uparrow$ &
     
     &{\# params} & {\# steps} &
     
     & \multicolumn{2}{c}{{CAS $\times 100$} $\uparrow$}  
     \\
     \cline{12-13}
    &&  && & &&& & && {Top-1 (76.6)} & {Top-5 (93.1)} \\[-7pt]
    \textbf{ImageNet 256$\times$256} && &&& &&& &&& &
    \\[-2pt]
    \midrule
    

     
    DCTransformer~\cite{nash2021generating} $^\square$ &
    & 36.51 & n/a &
    & 0.36 & \textbf{0.67} &
    & 738M & $>$1024 &   & &
     \\ 
    
    BigGAN-deep~\cite{biggan}  & %, 1.0 trunc. &
    & 6.95 & \bfseries{198.2} &
    & \textbf{0.87} & 0.28 &
    & 160M & 1 & & 43.99 &67.89 \\
    \\
    
    % Improved DDPM~\cite{nichol2021improved} &
    % & 31.5 &   &
    % & ?0.70 & ?0.62 &
    % &  & &
    % & 270M & 250 \\
    Improved DDPM~\cite{nichol2021improved}$^\square$  &
    & 12.26 & n/a  &
    & 0.70 & 0.62 &
     & 280M & 250  &  &  & \\
    
    ADM~\cite{dhariwal2021diffusion}$^\square$   & 
    & 10.94 & 101.0  &
    & 0.69 & 0.63 &
    & 554M & 250 &  &  & \\
    
    % ADM-G, 1.0 guid. & 
    % & 4.59 & 186.7  &
    % & ?0.69 & ?0.63 &
    % &  &  &
    % & 554M & 250  %554M + 54M classfier
    % \\

    
    VQVAE-2~\cite{Razavi19vqvae2}$^\square$ &
    & 31.11 & $\sim$45 &
    & 0.36 & 0.57 &
    & 13.5B$^{\blackdiamond}$ & 5120 & & 54.83 & 77.59 \\
   % \midrule
   % \bfseries{\model Baseline} && 18.98 & 192.52 && ? & ? && ?? & ?? \\
    \midrule
    VQ-GAN~\cite{Esser21vqgan}$^\square$ &
    
    & 15.78 & 78.3 &
    & n/a & n/a &
    & 1.4B & 256 &  &  &
    \\
 
    VQ-GAN$^\ast$ &
    & 18.65 & 80.4 &
    & 0.78 & 0.26 &
    & 227M & 256 & 
    & 53.10 $^\dagger$ & 76.18 $^\dagger$
     \\
 &
    & & &
    & & &
    &  & & 
    & 47.50 & 68.90
     \\
    % VQ-GAN, 0.05 RS &
    % & 1.4B +  & 5120 &
    % & 5.20 & 380.3 &
    % % & ? & ? &
    % &  & \\
%     \bfseries{\model-Linear} &
    
%     &  &  &
%     &  &  &
%   & 227M  & 16 &
%      & &
   
    \bfseries{\model (Ours)} &
    
    & \bfseries{\bestfid} & \bestis &
    & 0.80 & 0.51 &
   & 227M  & 8 &
   & \bfseries{63.14}$^\dagger$ & \bfseries{84.45}$^\dagger$ 
    \\
    &&  & &
    & & &
   & & &
   & 58.20 & 79.65
    \\
    % 227M + 54M
    % \bfseries{Ours, 0.05 RS} &
    % & +  &  &
    % & 5.90 & 152.9 &
    % % & ? & ? &
    % &  &  \\

   
    % Validation &
    % &- & - &
    % & 1.62 & 234.0  &
    % % & ? & ? &
    % &  73.09 &  91.47 \\
    \bottomrule
    \\[-4pt]
    \textbf{ImageNet 512$\times$512} && &&& &&& &&& &\\[-2pt]
    \midrule
    
     BigGAN-deep~\cite{biggan} & & 8.43 & \bfseries{232.5} & & \textbf{0.88} & 0.29 &
     &160M&1&&44.02&68.22
     \\
     
     ADM~\cite{dhariwal2021diffusion}$^\square$ & & 23.24 & 58.06 &&0.73& \textbf{0.60} & 
     &559M&250&
     && \\
    %  ADM, 1.0 guid. & 7.72 & & 0.87 & 0.42  \\
     \midrule
     VQGAN$^\ast$ & & 26.52 & 66.8 &
     & 0.73 & 0.31 &
      & 227M &1024 &
      &51.29&74.24 \\
     \bfseries{\model (Ours)} & & \bfseries{\bestfidhighres} & 156 & &  0.78 & 0.50 & & 227M &12&
     &63.43&84.79 \\
     % \bfseries{Ours}, 0.5 RS & ? & ? & &  \\
    \bottomrule
    
    \end{tabular}
    }
    \vspace{-5pt}
    \caption{Quantitative comparison with state-of-the-art generative models on ImageNet 256$\times$256 and 512$\times$512. 
    %
    \footnotesize{``\# steps” refers to the number of neural network runs needed to generate a sample.  $^\ast$ denotes the model we train with the same architecture and setup with ours; $^\square$ denotes values taken from prior publications; $^\blackdiamond$ estimated based on the pytorch implementation~\cite{pytorch2020vqvae2}. The CAS score is computed on the converged model trained for 300 epochs where $^\dagger$ indicates the model trained with strong data augmentation Randaugment~\cite{cubuk2020randaugment}.} 
    }
    \label{tab:maintable}
    % On average 10-15ms per step

\end{table*}

==> figures/class_cond_visual_4x4.tex <==
\newcommand{\tmpwidth}{0.24\linewidth}
\setlength{\tabcolsep}{2pt}
\begin{figure*}[!ht]
    \centering
    \begin{tabular}{c c c c}
     \includegraphics[width=\tmpwidth]{figures/diversity4x4/000_4x4_biggan.png}&
    \includegraphics[width=\tmpwidth]{figures/diversity4x4/000_4x4_vqvae2.png}&
    \includegraphics[width=\tmpwidth]{figures/diversity4x4/000_4x4_ours8.png}&
    \includegraphics[width=\tmpwidth]{figures/diversity4x4/000_4x4_ours64.png} \\
     \includegraphics[width=\tmpwidth]{figures/diversity4x4/001_4x4_biggan.png}&
    \includegraphics[width=\tmpwidth]{figures/diversity4x4/001_4x4_vqvae2.jpg}&
    \includegraphics[width=\tmpwidth]{figures/diversity4x4/001_4x4_ours8.png}&
    \includegraphics[width=\tmpwidth]{figures/diversity4x4/001_4x4_ours64.png} \\
     \includegraphics[width=\tmpwidth]{figures/diversity4x4/009_4x4_biggan.png}&
    \includegraphics[width=\tmpwidth]{figures/diversity4x4/009_4x4_vqvae2.jpg}&
    \includegraphics[width=\tmpwidth]{figures/diversity4x4/009_4x4_ours8.png}&
    \includegraphics[width=\tmpwidth]{figures/diversity4x4/009_4x4_ours64.png} \\
    BigGAN-deep (FID=$6.95$) & VQVAE-2 (FID=31.11) &  \model-8 (FID=\bestfid) &  \model-64 (FID=5.14) \\
    \end{tabular}
    \vspace{-2mm}
    
    \caption{Sample Diversity Comparison between BigGAN-deep~\cite{biggan}, VQVAE-2\cite{Razavi19vqvae2}, and our proposed method \model on ImageNet 256$\times$256.
    %BigGAN was sampled with $1.0$ truncation to yield the maximum diversity. In contrast to BigGAN's samples, our proposed method generate more diverse samples such as varied lighting, poses, scales and context, which are visually closer to the training set.
    The class ids of the samples from top to bottom are {\footnotesize{ \texttt{000}}, \footnotesize{\texttt{001}}, and \footnotesize{\texttt{009}}} respectively. VQVAE-2 and BigGAN
samples are taken from VQVAE-2\cite{Razavi19vqvae2}. Please refer to appendix for more comparisons.}
    \vspace{-4mm}
    \label{fig:diversity}
\end{figure*}

==> figures/editing.tex <==

\renewcommand{\tmpwidth}{0.14\linewidth}
\setlength{\tabcolsep}{1pt}
\begin{figure*}[!ht]
    \centering
    \begin{tabular}{c c c c c c c}

	% \includegraphics[width=\tmpwidth]{figures/editing/000143_to130_0020_input.png} & 
	\includegraphics[width=\tmpwidth]{figures/editing/000193_to282_0006_input.png} &
	\includegraphics[width=\tmpwidth]{figures/editing/000689_to282_0000_input.png} &
	\includegraphics[width=\tmpwidth]{figures/editing/000838_to282_0004_input.png} &
	\includegraphics[width=\tmpwidth]{figures/editing/000538_to282_0024_input.png} &
	\includegraphics[width=\tmpwidth]{figures/editing/000018_to282_0002_input.png} &
	\includegraphics[width=\tmpwidth]{figures/editing/000809_to282_0002_input.png} &
	\includegraphics[width=\tmpwidth]{figures/editing/000985_to282_0000_0024_input.png} 
    \\ 
	% \includegraphics[width=\tmpwidth]{figures/editing/000143_to130_0020_output.png} & 
	\includegraphics[width=\tmpwidth]{figures/editing/000193_to282_0006_output.png} &
	\includegraphics[width=\tmpwidth]{figures/editing/000689_to282_0000_output.png} &
	\includegraphics[width=\tmpwidth]{figures/editing/000838_to282_0004_output.png} &
    \includegraphics[width=\tmpwidth]{figures/editing/000538_to282_0036_output.png} &
    \includegraphics[width=\tmpwidth]{figures/editing/000018_to282_0000_output.png} &
	\includegraphics[width=\tmpwidth]{figures/editing/000809_to282_0002_output.png} &
    \includegraphics[width=\tmpwidth]{figures/editing/000985_to282_0000_0012_output.png} 
    \\
    \end{tabular}
    \caption{\textbf{Object modification.} Given input images in the first row, and a target class "tiger cat", \model replaces the bounding boxed regions with tiger cats. The fact that the synthesized tiger cat blends in with the rest of the image seamlessly highlights the composition ability of our model.  \todo{add bounding box}}
    \vspace{-6mm}
    \label{fig:editing}
\end{figure*}

==> figures/rebuttal_table1.tex <==

\setlength{\tabcolsep}{2pt}
\begin{table}[h]
\small
    \centering
    
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{l lc cc c cc}
        \toprule
        &&& \multicolumn{2}{c}{ImageNet256x256} && \multicolumn{2}{c}{ImageNet512x512}  \\\cline{4-5} \cline{7-8}
 Model & Classifier guidance && FID & IS && FID & IS            \\ 
\midrule
% ADM~[9]  & & & 23.24& 58.06 && 10.94 & 101.0  \\
% % VQ-GAN~[11]       & & & n/a & n/a && 15.78 & 78.3  \\
% VQGAN\cite{Esser21vqgan} & & & 26.52$^\ast$ & 66.18$^\ast$ && 15.78 & 78.3 \\
% MaskGIT                         & & & 7.32 & 156.0 && 6.18 & 182.1 \\ \cline{2-8}

ADM~\cite{dhariwal2021diffusion}  & 1.0 guidance  && 4.59 & 186.70  && 7.72 & 172.71 \\
VQGAN~\cite{Esser21vqgan} & 0.05 acceptance rate    &&  5.88 & 304.8 && n/a  & n/a \\
MaskGIT & 0.05 acceptance rate    &          & \textbf{4.02} & \textbf{355.6} && \textbf{4.46} & \textbf{342.0} \\
  \bottomrule
    \end{tabular}
    
    }
    \vspace{-3mm}
    \caption{\small{Class-conditional image synthesis on ImageNet for methods with classifier guidance.}}
    \label{tab:supp_cc_classifier}
\vspace{-3mm}
\end{table}


% \setlength{\tabcolsep}{4pt}
% \begin{table}[t]
% \small
%     \centering
%     {\small
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{ll ccccc}
% \toprule
% Dataset & Model &  FID & IS & Precision & Recall & \# Steps \\
% \midrule
% ImageNet & ADM\cite{dhariwal2021diffusion} & 23.24 & 58.06 & 0.73 & 0.60 & 250 \\
% 512x512 & MaskGIT \cite{dhariwal2021diffusion} & 7.32 & 156.0 & 0.78 & 0.50 & 12 \\
%  \cline{2-7}
% & ADM guid.\cite{dhariwal2021diffusion} & 7.72 & 172.71 & \textbf{0.87} & 0.42 & 250 \\
% & MaskGIT guid.$^\blackdiamond$ & \textbf{4.46} & \textbf{342.0} & 0.83 & \textbf{0.44} & 240 \\
%  \cline{2-7}
% & ADM guid. + ADM upsa. & \textbf{3.83} & 221.72 & 0.84 & 0.53 & 500 \\
% \midrule
% ImageNet 
% & ADM guid.\cite{dhariwal2021diffusion} & 4.59 & 186.70 & 0.82 & \textbf{0.52} & 250 \\
% 256x256 & VQGAN guid.\cite{Esser21vqgan}$^\blackdiamond$ & 5.88 & 304.8 & n/a & n/a & 5120\\
% & MaskGIT guid.$^\blackdiamond$ & \textbf{4.02} & \textbf{355.6} & \textbf{0.83} & 0.50 & 200 \\
%  \cline{2-7}
% & ADM guid + ADM upsa. & \textbf{3.94} & 215.84 & 0.83 & 0.53 & 500 \\
%   \bottomrule
%     \end{tabular}
%     }
%     }
%     \vspace{-.1cm}
%     \caption{\small{Class-conditional ImageNet comparison for methods with classifier guidance. \small{$^\blackdiamond$ represents with classifier guidance using rejection sampling with 0.05 acceptance rate as in VQGAN\cite{Esser21vqgan}.}}}
%     \label{tab:classifier}
% \vspace{-2mm}
% \end{table}

==> figures/scheduling.tex <==
% \begin{table}[htbp]
% 	\centering
% 	 \begin{tabular}{c | l  c  c }
% 	 \multirow{5}{*}{
%       \begin{minipage}{.3\textwidth}
%       \includegraphics[width=\linewidth]{figures/scheduling.pdf}
%     \end{minipage}
%     }
% 	% \vspace{-6mm}
%     & \mathbf{f} & FID & IS \\
%   \cline{2-4}
% 	& uniform & & \\
% 	& $x^2$ & & \\
% 	& $x^3$ & & \\
% 	& $x^0.5$ & & \\
% 	& cosine & & \\
% 	& log &&  \\
% 	& exp && \\

% 	\end{tabular}
% 		\caption{Scheduling}
% 	\label{table:scheduling}
% \end{table}
\begin{figure}
	\centering
      \includegraphics[width=0.8\linewidth]{figures/scheduling.pdf}
		\caption{\textbf{Choices of Mask Scheduling Functions} $\gamma (\frac{t}{T})$.}
		%$n = \lceil \mathbf{r}(\frac{t}{T}) N \rceil$}
	\label{fig:scheduling}
\end{figure}


==> figures/supp1_class_cond_diversity.tex <==
\newcommand{\tmpwidth}{0.33\linewidth}

\begin{figure*}[!ht]
    \centering
    \begin{tabular}{c c c c}

    
    \includegraphics[ width=\tmpwidth]{figures/diversity/130_biggan_trun1.png} & \hspace{-3mm}
    \includegraphics[ width=\tmpwidth]{figures/diversity/130_ours.png} & \hspace{-3mm}
    \includegraphics[ width=\tmpwidth]{figures/diversity/130_gt.png} \\ 
    
    \includegraphics[ width=\tmpwidth]{figures/diversity/145_biggan_trun1.png} & \hspace{-3mm}
    \includegraphics[ width=\tmpwidth]{figures/diversity/145_ours.png} & \hspace{-3mm}
    \includegraphics[ width=\tmpwidth]{figures/diversity/145_gt.png} \\
    
    \includegraphics[ width=\tmpwidth]{figures/diversity/000_biggan_trun1.png} & \hspace{-3mm}
    \includegraphics[ width=\tmpwidth]{figures/diversity/000_ours1.png} & \hspace{-3mm}
    \includegraphics[ width=\tmpwidth]{figures/diversity/000_gt.png} \\   
    
    BigGAN-deep (FID=$6.95$) & \model (FID=\bestfid) & Training Set \\
    \end{tabular}
    \caption{More Sample Diversity Comparisons for BigGAN-deep with truncation $1.0$ and our proposed method \model on ImageNet.}
    % \vspace{-6mm}
    \label{fig:supp_diversity}
\end{figure*}

==> figures/supp_class_cond_maskgit64.tex <==
\renewcommand{\tmpwidth}{36mm}
\newcommand{\tmpheight}{72mm}
\setlength{\tabcolsep}{2pt}
\begin{figure*}[!ht]
    \centering
    \begin{tabular}{c c c c}

   
    BigGAN (FID=$6.95$) & VQVAE-2$^\dagger$ (FID=$31$) & \model-8 (FID=\bestfid) & \model-64 (FID=5.14) \\
    \includegraphics[width=\tmpwidth,  height=\tmpheight]{figures/supp_cc/22_bald-eagle_biggan.jpg} & 
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/22_bald-eagle_vqvae2.jpg} & 
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/22_bald-eagle_vqgan.jpg} & \ 
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/22_bald-eagle_ours.png} &
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/22_bald-eagle_ours64.png}\\ 
       
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/108_anemone_biggan.jpg} & \
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/108_anemone_vqvae2.jpg}& \
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/108_anemone_vqgan.jpg} & \ 
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/108_anemone_ours.png} &
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/108_anemone_ours64.png}\\ 
    
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/97_drake_biggan.jpg} & \
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/97_drake_vqvae2.jpg}& \
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/97_drake_vqgan.jpg} & \ 
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/97_drake_ours.png} & 
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/97_drake_ours64.png}\\ 
        
    \end{tabular}
    \caption{\textbf{More diversity comparisons} between BigGAN-deep with truncation $1.0$, VQVAE-2\cite{vqvae2}, and our proposed method \model on ImageNet. $^\dagger$ represents extracted samples from the paper.}
    \vspace{-6mm}
    \label{fig:supp_cc_diversity0}
\end{figure*}
    
\begin{figure*}[!ht]
    \centering
    \begin{tabular}{c c c c}
    BigGAN (FID=$6.95$) & VQVAE-2$^\dagger$ (FID=$31$) & \model-8 (FID=\bestfid) & \model-64 (FID=5.14) \\
    
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/0_tench_biggan.jpg} & \
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/0_tench_vqvae2.jpg}& \
    % % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/0_tench_vqgan.jpg} & \ 
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/0_tench_ours.png} \\ 

    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/1_goldfish_biggan.jpg} & \
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/1_goldfish_vqvae2.jpg}& \
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/1_goldfish_ours.png} \\ 
    
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/141_redshank_biggan.jpg} & \
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/141_redshank_vqvae2.jpg}& \
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/141_redshank_vqgan.jpg} & \ 
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/141_redshank_ours.png} &
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/141_redshank_ours64.png}\\ 
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/154_biggan.png} & \
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/154_vqvae2.png}& \
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/141_redshank_vqgan.jpg} & \ 
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/154_ours8.png} &
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/154_ours64.png}\\ 

    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/130_flamingo_biggan.png} & \
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/130_flamingo_vqvae2.png}& \
    % \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/141_redshank_vqgan.jpg} & \ 
    
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/130_flamingo_ours8.png} &
    \includegraphics[ width=\tmpwidth, height=\tmpheight]{figures/supp_cc/130_flamingo_ours64.png} \\ 
\end{tabular}
    \caption{More Diversity Comparisons among BigGAN-deep with truncation $1.0$, VQVAE-2\cite{vqvae2}, and our proposed method \model on ImageNet. $^\dagger$ represents extracted samples from the paper.}
    \vspace{-6mm}
    \label{fig:supp_cc_diversity2}
\end{figure*}

==> figures/uncrop_comparison.tex <==

\renewcommand{\tmpwidth}{0.25\linewidth}
\setlength{\tabcolsep}{1pt}
\begin{figure}[!ht]
    \centering
    \begin{tabular}{cccc}
    \includegraphics[width=\tmpwidth]{figures/uncrop/001704_input.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/3101_boundless.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/3101_inf.png}&
    \includegraphics[width=\tmpwidth]{figures/uncrop/3101_ours.png} &
    \includegraphics[width=\tmpwidth]{figures/uncrop/3101_output2.png} &
    \includegraphics[width=\tmpwidth]{figures/uncrop/3101_output4.png} 
   % \includegraphics[width=\tmpwidth]{figures/uncrop/3101_gt.png} 
    \\
%      \includegraphics[width=\tmpwidth]{figures/uncrop/3101_input.png}&
%     % \includegraphics[width=\tmpwidth]{figures/uncrop/3101_boundless.png}&
%     % \includegraphics[width=\tmpwidth]{figures/uncrop/3101_inf.png}&
%     \includegraphics[width=\tmpwidth]{figures/uncrop/3101_ours.png} &
%     \includegraphics[width=\tmpwidth]{figures/uncrop/3101_output2.png} &
%     \includegraphics[width=\tmpwidth]{figures/uncrop/3101_output4.png} 
%   % \includegraphics[width=\tmpwidth]{figures/uncrop/3101_gt.png} 
%     \\
    
    % \includegraphics[width=\tmpwidth]{figures/uncrop/2982_input.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/2982_boundless.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/2982_inf.png}&
    
    % \includegraphics[width=\tmpwidth]{figures/uncrop/2982_output5.png} &
    % \includegraphics[width=\tmpwidth]{figures/uncrop/2982_output0.png} &
    % %\includegraphics[width=\tmpwidth]{figures/uncrop/2982_output9.png} &
    % \includegraphics[width=\tmpwidth]{figures/uncrop/2982_output3.png} &
    % % \includegraphics[width=\tmpwidth]{figures/uncrop/2982_output13.png} &
    % \includegraphics[width=\tmpwidth]{figures/uncrop/2982_gt.png}  \\
    
    \includegraphics[width=\tmpwidth]{figures/uncrop/3996_input.png}&
    %\includegraphics[width=\tmpwidth]{figures/uncrop/3996_boundless.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/3996_inf.png}&
    \includegraphics[width=\tmpwidth]{figures/uncrop/3996_output8.png} &
    \includegraphics[width=\tmpwidth]{figures/uncrop/3996_output1.png} &
    \includegraphics[width=\tmpwidth]{figures/uncrop/3996_output9.png} 
    %\includegraphics[width=\tmpwidth]{figures/uncrop/3996_gt.png}
   \\
    % \includegraphics[width=\tmpwidth]{figures/uncrop/3145_input.png}&
    % % \includegraphics[width=\tmpwidth]{figures/uncrop/3145_boundless.png}&
    % % \includegraphics[width=\tmpwidth]{figures/uncrop/3145_inf.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/3145_output7.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/3145_output1.png}&
    % %\includegraphics[width=\tmpwidth]{figures/uncrop/3145_output2.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/3145_output6.png}&
    % % \includegraphics[width=\tmpwidth]{figures/uncrop/3145_gt.png}
    % \\
   
    % Input & Boundless & InfinityGAN\footnotesize{\ding{83}}  & \multicolumn{3}{c}{------ \model (Our Samples) ------} & Groundtruth \\
    
    \includegraphics[width=\tmpwidth]{figures/uncrop/harley-davidson-xAHtaYIHlPI_input_0.png}&
    %\includegraphics[width=\tmpwidth]{figures/uncrop/2142_003_hifill.png}&
    %\includegraphics[width=\tmpwidth]{figures/uncrop/2142_003_hifill.png}&
    %\includegraphics[width=\tmpwidth]{figures/uncrop/2142_003_output12.png}&
    \includegraphics[width=\tmpwidth]{figures/uncrop/harley-davidson-xAHtaYIHlPI_output_12.png}&
    \includegraphics[width=\tmpwidth]{figures/uncrop/harley-davidson-xAHtaYIHlPI_output_03.png}&
    \includegraphics[width=\tmpwidth]{figures/uncrop/harley-davidson-xAHtaYIHlPI_output_06__.png}
    %\includegraphics[width=\tmpwidth]{figures/uncrop/2142_003_gt.png}
    \\
    
    % \includegraphics[width=\tmpwidth]{figures/uncrop/7480_003_input.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/7480_003_hifill.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/7480_003_hifill.png}&
    % %\includegraphics[width=\tmpwidth]{figures/uncrop/2142_003_output12.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/7480_003_output0.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/7480_003_output2.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/7480_003_output6.png}&
    % \includegraphics[width=\tmpwidth]{figures/uncrop/7480_003_gt.png} \\   
    Input  & \multicolumn{3}{c}{------ \model (Our Samples) ------} \\    
    % Input & DeepFill & HiFill  & \multicolumn{3}{c}{------ \model (Our Samples) ------} & Groundtruth \\    
    \end{tabular}
    \vspace{-3mm}
    \caption{\textbf{Inpainting and outpainting.} Given a single input image (leftmost column), \model synthesizes diverse results for outpainting with different directions and inpainting tasks. (columns to the right). }
    \vspace{-6mm}
    \label{fig:uncrop_diversity}
\end{figure}



==> figures/uncrop_table.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\small
    \centering
    {\small
    \begin{tabular}{llc ccc}
    \toprule
    {Task} & {Model} &
    & {FID}  $\downarrow$ & {IS} $\uparrow$ & %{L1} $\downarrow$ 
   % {Fool Rate} $\uparrow$ 
    \\
    \midrule
    \textit{\textbf{Outpainting}}
    & 
    Boundless \cite{teterwak2019boundless}$^{\square}$ & 
    & 35.02 & 6.15 & 
    %.064%
    \\
        
    % NS-Outpaint \cite{}$^{\square}$ &
    % & 50.68 & 4.70 &   \\   
    
     {\footnotesize Right 50\%} & In\&Out \cite{cheng2021inout}$^{\square}$ &
    & 23.57 & 7.18 &  \\
    

    & InfinityGAN \cite{lin2021infinitygan} &
    & 10.60 & 5.57 &
    \\
    
    & Boundless \cite{teterwak2019boundless} TF $^{\blackdiamond}$ & 
    & 7.80 & 5.99 &
    %.064% 
    \\
     
    & \textbf{\model (Ours)} $^{512}$& 
    & \textbf{6.78} & \textbf{11.69} &  \\[2pt]
    \midrule
    \textit{\textbf{Inpainting}} & 
     DeepFill \cite{yu2019free} &
    & 11.51 & 22.55 & \\
    
 {\footnotesize Center 50\%$\times$50\%} & HiFill \cite{yi2020contextual}$^{512}$ & 
    & 16.60 & 19.93 &  \\
    
    & \textbf{\model (Ours)$^{512}$} &
    & \textbf{7.92} & \textbf{22.95} & \\
    \bottomrule
    \end{tabular}
    }
    % \vspace*{0.35cm}
    \caption{Quantitative Comparison for Inpainting and Outpainting on the Places2 dataset. \footnotesize{$^{512}$ evaluated on 512$\times$512 samples while other work evaluated on the corresponding 256$\times$256 ones, consistent with their training; $^\square$ taken from the prior work. $^\blackdiamond$ evaluated using the TFHub model\cite{boundless_tfhub}.} }
    \label{tab:inpaint_uncrop}
\vspace{-6cm}
\end{table}





% \setlength{\tabcolsep}{3pt}
% \begin{table}[h]
% \small
%     \centering
%     {\small
%     \begin{tabular}{llc cccc}
%     \toprule
%     {Task} & {Model} &
%     & {FID}  $\downarrow$ & {Lpips}  $\downarrow$ & {User Study} $\uparrow$ \\
%     \midrule
%     \textit{Outpainting} & Boundless \cite{teterwak2019boundless} & 
%     & 20.8 & 0.29 & ??  \\
    
%     & InfinityGAN \cite{lin2021infinitygan} &
%     & 18.5 &\textbf{0.28} & ??  \\
    
%     & \textbf{\model (Ours)}& 
%     & \textbf{7.3} & 0.32 & \textbf{??} \\
%     \midrule
%     \textit{Inpainting} & DeepFill \cite{yu2019free} &
%     & 14.3 & ?? & ?? \\
    
%     & HiFill \cite{yi2020contextual} & 
%     & 15.9 & 0.21 & ?? \\
    
%     & \textbf{\model (Ours)} &
%     & \textbf{10.9} &\textbf{0.25} & \textbf{??} \\
    
%     \bottomrule
%     \end{tabular}
%     }
%     % \vspace*{0.35cm}
%     \caption{Quantitative Comparison for Inpainting and Outpainting.}
%     \label{tab:inpaint_uncrop}
% \vspace{-.2cm}
% \end{table}

==> figures/why_masking_scheduling.tex <==
\begin{figure}[!t]
    \centering
	\includegraphics[width=\linewidth]{figures/why_masking.pdf}
    \vspace{-5mm}
    \caption{\textbf{Motivation for refinement scheduling}. Given each image with a varying percentage of their visual tokens masked out, the trained \model is tasked with completing the remaining tokens. Note the abrupt global change from  90\% to 95\%.\lu{I found this figure confusing. Why it suddenly change everything at the last 5\%. This is kind of against the example you have in Figure 1 and the general story. We should consider removing it if it is only used to show why masking is important. (after ddl we should talk about this behavior more.)}}
    \label{fig:why_masking}
\end{figure}
